Normalized neural representations of natural odors

The olfactory system removes correlations in natural odors using a network of inhibitory neurons in the olfactory bulb. It has been proposed that this network integrates the response from all olfactory receptors and inhibits them equally. However, how such global inhibition influences the neural representations of odors is unclear. Here, we study a simple statistical model of this situation, which leads to concentration-invariant, sparse representations of the odor composition. We show that the inhibition strength can be tuned to obtain sparse representations that are still useful to discriminate odors that vary in relative concentration, size, and composition. The model reveals two generic consequences of global inhibition: (i) odors with many molecular species are more difficult to discriminate and (ii) receptor arrays with heterogeneous sensitivities perform badly. Our work can thus help to understand how global inhibition shapes normalized odor representations for further processing in the brain.

==> common.tex <==
% This file defines common macros used in many LaTeX files.
% They are collected here for convenience use.

% packages
\usepackage{amsmath}
\usepackage{xcolor}
\usepackage{dsfont} % double stroke font
\usepackage{xspace}


% abbrevations - use \mbox instead of \nolinebreak since this works in captions, too
\newcommand{\ie}{\mbox{i.\hspace{0.125em}e.}\@\xspace}
\newcommand{\eg}{\mbox{e.\hspace{0.125em}g.}\@\xspace}
\newcommand{\etal}{\mbox{et al.}\@\xspace}
\newcommand{\kb}{k_{\rm B}}
\newcommand{\kB}{k_{\rm B}}
\newcommand{\kbT}{k_{\rm B}T}
\newcommand{\kBT}{k_{\rm B}T}
\newcommand{\const}{\text{const.}}

% colors, which are often used
\definecolor{plot1}{RGB}{6,115,183}
\definecolor{plot2}{RGB}{255,118,0}
\definecolor{plot3}{RGB}{0,169,25}
\definecolor{plot4}{RGB}{230,0,28}
\definecolor{plot5}{RGB}{0,0,0}
\definecolor{plotBlue}{RGB}{6,115,183}
\definecolor{plotOrange}{RGB}{255,118,0}
\definecolor{plotGreen}{RGB}{0,169,25}
\definecolor{plotRed}{RGB}{230,0,28}

% draft commands
\newcommand{\fixme}[1]{\textcolor{red}{FIXME: #1}}
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\edit}[1]{\textcolor{blue}{#1}}

% references - use \mbox instead of \nolinebreak since this works in captions, too
\newcommand{\Eqref}[1]{\mbox{Eq.\hspace{0.25em}\eqref{#1}}}
\newcommand{\Eqsref}[1]{\mbox{Eqs.\hspace{0.25em}\eqref{#1}}}
\newcommand{\figref}[1]{\mbox{Fig.\hspace{0.25em}\ref{#1}}}
\newcommand{\figsref}[1]{\mbox{Figs.\hspace{0.25em}\ref{#1}}}
\newcommand{\refcite}[1]{\mbox{Ref.\hspace{0.25em}\cite{#1}}}

% math constructs
\newcommand{\im}{{\mathbf{i}}}
\newcommand{\diff}{\text{d}}
\newcommand{\pfrac}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\deltafrac}[2]{\frac{\delta #1}{\delta #2}}
\newcommand{\difffrac}[2]{\frac{\diff #1}{\diff #2}}
\newcommand{\takenat}[2]{\left.{#1}\right|_{#2}}
\newcommand{\abs}[1]{|{#1}|}
\newcommand{\Abs}[1]{\left| {#1} \right|}
\newcommand{\order}[1]{\mathcal{O}(#1)}
\newcommand{\Order}[1]{\mathcal{O}\left(#1\right)}
\newcommand{\set}[1]{\{{#1}\}}
\newcommand{\Set}[1]{\left\{{#1}\right\}}
\newcommand{\unity}{\mathds{1}}
\newcommand{\transpose}[1]{{#1}^\top}
\newcommand{\scalarproduct}[2]{\langle #1 ,\, #2 \rangle}
\newcommand{\Scalarproduct}[2]{\left\langle #1 ,\, #2 \right\rangle}

% math font sizes
\newcommand{\msmall}[1]{\mbox{\small $#1$}}
\newcommand{\mscriptsize}[1]{\mbox{\scriptsize $#1$}}
\newcommand{\mtiny}[1]{\mbox{\tiny $#1$}}

%\newcommand{smallequation}[1]{\begingroup\small#1\endgroup}
\newenvironment{smallequation}{\begingroup\small\ignorespaces}{\endgroup\ignorespacesafterend}

% math sets
\newcommand{\natnum}{\mathds{N}}
\newcommand{\integers}{\mathds{Z}}
\newcommand{\rationals}{\mathds{Q}}
\newcommand{\reals}{\mathds{R}}
\newcommand{\complexes}{\mathds{C}}

% math operators
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\sgn}{sgn}
%\DeclareMathOperator{\max}{max}
%\DeclareMathOperator{\min}{min}
\DeclareMathOperator{\std}{std}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\CV}{Cv}
\DeclareMathOperator{\STD}{STD}
\DeclareMathOperator{\SEM}{SEM}
\DeclareMathOperator{\erf}{erf}
\DeclareMathOperator{\erfc}{erfc}
\newcommand{\mean}[1]{\langle #1 \rangle}
\newcommand{\Mean}[1]{\left\langle #1 \right\rangle}
\renewcommand\Re{\operatorname{\mathfrak Re}}
\renewcommand\Im{\operatorname{\mathfrak Im}}
\newcommand{\Floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\Ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\Nabla}{\vect\nabla}

% special words
\newcommand{\gene}[1]{\mbox{\textit{#1}}}

% special symbols
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{<-> mathx10}{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareMathAccent{\widebar}{0}{mathx}{"73}
\newcommand{\vect}{\boldsymbol}
\newcommand{\mat}[1]{\underline{\underline{#1}}}

% symbols for perturbation analysis
\newcommand{\eps}{\varepsilon}
\newcommand{\pert}{\widehat}
\newcommand{\steady}[1]{\widebar{#1}}
\newcommand{\pprime}{\prime\prime}
\newcommand{\ppprime}{\prime\prime\prime}

% roman numbers with bars
\def\barroman#1{\sbox0{#1}\dimen0=\dimexpr\wd0+1pt\relax
  \makebox[\dimen0]{\rlap{\vrule width\dimen0 height 0.06ex depth 0.06ex}%
    \rlap{\vrule width\dimen0 height\dimexpr\ht0+0.03ex\relax 
            depth\dimexpr-\ht0+0.09ex\relax}%
    \kern.5pt#1\kern.5pt}}
 
  
% hyphenation

\hyphenation{non-equilibrium}



